Spotting Silent Buffer Overflows in Execution Trace through Graph Neural Network Assisted Data Flow Analysis

A software vulnerability could be exploited without any visible symptoms. When no source code is available, although such silent program executions could cause very serious damage, the general problem of analyzing silent yet harmful executions is still an open problem. In this work, we propose a graph neural network (GNN) assisted data flow analysis method for spotting silent buffer overflows in execution traces. The new method combines a novel graph structure (denoted DFG+) beyond data-flow graphs, a tool to extract {\tt DFG+} from execution traces, and a modified Relational Graph Convolutional Network as the GNN model to be trained. The evaluation results show that a well-trained model can be used to analyze vulnerabilities in execution traces (of previously-unseen programs) without support of any source code. Our model achieves 94.39\% accuracy on the test data and successfully locates 29 out of 30 real-world silent buffer overflow vulnerabilities. Leveraging deep learning, the proposed method is, to our best knowledge, the first general-purpose analysis method for silent buffer overflows. It is also the first method to spot silent buffer overflows in global variables, stack variables, or heap variables without crossing the boundary of allocated chunks.

==> floating.tex <==
\lstset{
language=[x32]Assembler,
stringstyle=\color{black},
keywordstyle=\color{black},
% xleftmargin=-.10\columnwidth, 
% xrightmargin=.10\columnwidth,
}
% \begin{minipage}{.95\columnwidth}
\begin{lstlisting}[caption={A case of float instruction},label=code:float,captionpos=b]
    ...
    mov 0x8(%ebp) %eax
    prefetcht2 (%edi)
    mov (%eax), %ecx
    ...
\end{lstlisting}
% \end{minipage}
% \begin{minipage}{.45\columnwidth}
% \begin{lstlisting}[caption={The Assemble Code Compiled from Source Code~\ref{code:sbof}},label=code:asm,captionpos=b]
%     ...
    
%     ...
% \end{lstlisting}
% \end{minipage}

==> graphs/strcpy.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{mygray}{gray}{0.9}

\lstset{
language=C,
frame=tb,
basicstyle={\small \bf \ttfamily}, %\scriptsize,\ttfamily,%
tabsize=3,
breaklines=true,
% breakatwhitespace=false,
showstringspaces=false,
% columns=fullflexible,
numbers=left,
numbersep=-10pt,                     % where to put the line-numbers
escapeinside={(*}{*)},
xleftmargin=2pt,
numberstyle=\small \bf \texttt, %\tiny, %\scriptsize,
stringstyle=\color{mauve},
keywordstyle= \color{black}, % \color{blue},
commentstyle=\color{dkgreen} \textit,%\scriptsize \textit,
}
\begin{lstlisting}[language=C++,
    directivestyle={\color{black}}
    emph={int,char,double,float,unsigned},
    emphstyle={\color{blue}},caption={Buffer overflow detection logic in ASAN's \texttt{strcpy}},label=code:sbof,captionpos=b]
    ...
    uptr from_size = REAL(strlen)(from) + 1;
    CHECK_RANGES_OVERLAP("strcpy", to, from_size, from, from_size);
    ASAN_READ_RANGE(ctx, from, from_size);
    ASAN_WRITE_RANGE(ctx, to, from_size);
    ...
\end{lstlisting}

==> sentence.tex <==
\section{Copied Sentence}
Reflection of the exact behavior of the program, optimizations and bugs in the compilers, unavailability of the source codes and platform-specific details are some reasons that make analyzing executable codes more preferable~\cite{balakrishnan2010wysinwyx}.

The objective of this work is to consider more of “semantic” definition of vulnerability patterns, based on some criteria that can be checked by means of lightweight static analysis, from binary code.
Note that similar views are also presented in~\cite{rawat2012finding}, but to the best of our knowledge, 
there is no implementation presented in applying deep learning to learning the semantic level informaiton so far.

Data flow patterns is manifold.

The the dataflow pattern could be extremly complex, 
an intuitive example can be find in one of Rawat's work~\cite{rawat2012finding}, 
they put lots of effort to indentify one kind of buffer overflow through static binary anaysis.
Despite the great efforts, they admit that \textsc{Boil} does not consider all the required features to 
trigger a buffer overflow vulnerability.
One of them is to ensure that \textit{the loop iteration condition is dependent on source buffer}.

Performing static analysis on binary code is challenging due to the lack of information usually available at the source level (e.g, type annotations)~\cite{rawat2012finding}
More recently, specific analysis have been developed for security purposes, like taint analysis [21], or string analysis [22].


Adjacent spatial safty violation
Non-adjacent spatial safty violation.
\url{https://github.com/microsoft/MSRC-Security-Research/blob/master/presentations/2019_02_BlueHatIL/2019_02%20-%20BlueHatIL%20-%20Trends%2C%20challenge%2C%20and%20shifts%20in%20software%20vulnerability%20mitigation.pdf}

We not only detect out-of-bound write, but also detect out-of-bound read.


given an image. 

hidden layer 1 will look like this (such things are viewed as a features by some researchers.). 

layer 2 will look like this.

features engineering.

-- SVM: (step 1) extrace the set of features; (step 2) using the extracted features to train a mode;

-- DNN: (step 1) original embedded: no need to extract explicit features; 
(step 2) a representation is learned;

